From Proof Nets to the Free *-Autonomous Category

In the first part of this paper we present a theory of proof nets for full multiplicative linear logic, including the two units. It naturally extends the well-known theory of unit-free multiplicative proof nets. A linking is no longer a set of axiom links but a tree in which the axiom links are subtrees. These trees will be identified according to an equivalence relation based on a simple form of graph rewriting. We show the standard results of sequentialization and strong normalization of cut elimination. In the second part of the paper we show that the identifications enforced on proofs are such that the class of two-conclusion proof nets defines the free *-autonomous category.

==> EdStraker.tex <==
%  macros for building up derivations ------------------------------------------

%                                                   +-------+--------+-------+
%                                                   |  dcl  |  dcc   |  dcr  |
%                                                   +-------+--------+-------+
%                                                       +---+        +---+
%                                                       | l |--------| m |
%                                                       +---+        +---+
%                                                             +----+
%                                                             | dc |
%                                                             +----+
%                                                   <---dl--->      <---dr--->
%
\newdimen\dercldim                                % dcl
\newdimen\derccdim                                % dcc
\newdimen\dercrdim                                % dcr
\newdimen\derldim                                 % dl
\newdimen\dercdim                                 % dc
\newdimen\derrdim                                 % dr
\newdimen\derdim                                  % d
\newdimen\derdldim                                % ddl
\newdimen\derdrdim                                % ddr
\newbox\derboxone                                 % b1
\newbox\derboxtwo                                 % b2
\newbox\derboxthree                               % b3
\newbox\derboxfour                                % b4
\newdimen\derquad\derquad=\fontdimen6\textfont2
\newdimen\deropen\deropen=\fontdimen5\textfont2\divide\deropen by3
\def\leaf #1{\global\setbox\derboxone=\hbox{\strut$#1$}%
   \global\derldim=0pt                            % dl=0
   \global\dercdim=\wd\derboxone                  % dc=wd(b1)
   \global\derrdim=0pt                            % dr=0
   }%
% \def\stem #1#2{%
%    \global\setbox\derboxone  =\hbox{\strut$\scriptstyle #1\;$}%
%    \global\setbox\derboxtwo  =\vbox{\offinterlineskip\hbox{$\|$}\hbox{$\|$}}%
%    \global\setbox\derboxthree=\hbox{\strut$\scriptstyle \;#2$}%
%    \global\derldim=\wd\derboxone                  % dl=wd(b1)
%    \global\dercdim=\wd\derboxtwo                  % dc=wd(b2)
%    \global\derrdim=\wd\derboxthree                % dr=wd(b3)
%    }%
\def\rootaux #1#2#3{\setbox\derboxtwo=\hbox{\unhbox\derboxone}%
                                                  % b2=b1
   \setbox\derboxthree=\hbox 
      {$\smash{\lower\fontdimen22\textfont2\hbox{$#1$}}$}%
                                                  % b3; l=wd(b3)
   \setbox\derboxfour=\hbox 
      {$\smash{\lower\fontdimen22\textfont2\hbox{$#2$}}$}%
                                                  % b4; m=wd(b4)
   \leaf{#3}%                                     % dl=0, dc=wd(b1), dr=0
   \derdim=\dercdim\advance\derdim by-\derccdim\divide\derdim by2 
                                                  % d=(dc-dcc)/2
   \global\derldim=\dercldim\global\advance\derldim by-\derdim
                                                  % dl=dcl-d
   \global\derrdim=\dercrdim\global\advance\derrdim by-\derdim
                                                  % dr=dcr-d
%    \ifdim\derldim>0pt\ifdim\derrdim<0pt
%       \global\advance\derldim by\derrdim          % dl>0>dr -> dl=dl+dr, dr=0
%       \global\derrdim=0pt
%    \fi\fi
%    \ifdim\derrdim>0pt\ifdim\derldim<0pt
%       \global\advance\derrdim by\derldim          % dr>0>dl -> dr=dr+dl, dl=0
%       \global\derldim=0pt
%    \fi\fi
   \deropen=\fontdimen5\textfont2\divide\deropen by3
   \setbox\derboxone=\hbox{\vbox{\offinterlineskip
         \hbox{\ifdim\derldim<0pt\kern-\derldim\fi
               \box\derboxtwo
               \ifdim\derrdim<0pt\kern-\derrdim\fi}%
         \kern\deropen
         \hbox{\ifdim\dercldim>\derldim
                  \ifdim\derldim>0pt\kern\derldim\fi
                  \else\kern\dercldim\fi
               \hbox to0pt{\hss\copy\derboxthree}%
               \vbox{\ifdim\derccdim>\dercdim\hsize=\derccdim
                                        \else\hsize=\dercdim \fi
                    \hrule height.2pt depth.2pt width\hsize}%
               \hbox to0pt{\copy\derboxfour\hss}%
               \ifdim\dercrdim>\derrdim
                  \ifdim\derrdim>0pt\kern\derrdim\fi
                  \else\kern\dercrdim\fi}%
         \kern\deropen
         \hbox{\ifdim\derldim>0pt\kern\derldim\fi
               \box\derboxone
               \ifdim\derrdim>0pt\kern\derrdim\fi}}}%
   \ifdim\derldim<0pt\global\derldim=0pt\fi       % dl=max(dl,0)
   \ifdim\derrdim<0pt\global\derrdim=0pt\fi       % dr=max(dr,0)
   \derdldim=\wd\derboxthree\advance\derdldim by-\dercldim
                                                  % ddl=l-dcl
   \derdrdim=\wd\derboxfour \advance\derdrdim by-\dercrdim
                                                  % ddr=m-dcr
   \ifdim\derdim<0pt
      \ifdim\derdldim<0pt
         \derdldim=0pt                            % d<0, ddl<0 -> ddl=0
      \fi
      \ifdim\derdrdim<0pt
         \derdrdim=0pt                            % d<0, ddr<0 -> ddr=0
      \fi
   \else
      \ifdim\derldim>0pt
         \ifdim\derdldim>-\derdim
            \advance\derdldim by\derdim           % d>=0, dl>0, ddl+d>0 -> 
         \else			                          %                    ddl=ddl+d
            \derdldim=0pt                         % d>=0, dl>0, ddl+d<=0 ->
         \fi                                      %                        ddl=0
      \else
         \advance\derdldim by\dercldim            % d>=0, dl=0 -> ddl=ddl+dcl
      \fi
      \ifdim\derrdim>0pt
         \ifdim\derdrdim>-\derdim
            \advance\derdrdim by\derdim           % d>=0, dr>0, ddr+d>0 -> 
         \else			                          %                    ddr=ddr+d
            \derdrdim=0pt                         % d>=0, dr>0, ddr+d<=0 ->
         \fi                                      %                        ddr=0
      \else
         \advance\derdrdim by\dercrdim            % d>=0, dr=0 -> ddr=ddr+dcr
      \fi
   \fi
   \global\setbox\derboxone=\hbox
      {\kern\derdldim\unhbox\derboxone\kern\derdrdim}%
   \global\advance\derldim by\derdldim            % dl=dl+ddl
   \global\advance\derrdim by\derdrdim            % dr=dr+ddr
   }%
\def\rootr #1#2#3#4{{#4}%
   \dercldim=\derldim
   \derccdim=\dercdim
   \dercrdim=\derrdim
   \rootaux{#1}{#2}{#3}}%
\def\rrootr #1#2#3#4#5{\derquad=\fontdimen6\textfont2
   {#4}%
           \dercldim  =\derldim
   \setbox\derboxtwo=\hbox{\unhbox\derboxone\kern\derquad}%
           \derccdim  =\dercdim
   \advance\derccdim by\derrdim
   \advance\derccdim by\derquad
   {#5}%
   \setbox\derboxone=\hbox{\unhbox\derboxtwo\unhbox\derboxone}%
   \advance\derccdim by\derldim
   \advance\derccdim by\dercdim
           \dercrdim  =\derrdim
   \rootaux{#1}{#2}{#3}}%
\def\rrrootr #1#2#3#4#5#6{\derquad=\fontdimen6\textfont2
   {#4}%
           \dercldim  =\derldim
   \setbox\derboxtwo=\hbox{\unhbox\derboxone\kern\derquad}%
           \derccdim  =\dercdim
   \advance\derccdim by\derrdim
   \advance\derccdim by\derquad
   {#5}%
   \setbox\derboxtwo=\hbox{\unhbox\derboxtwo\unhbox\derboxone\kern\derquad}%
   \advance\derccdim by\derldim
   \advance\derccdim by\dercdim
   \advance\derccdim by\derrdim
   \advance\derccdim by\derquad
   {#6}%
   \setbox\derboxone=\hbox{\unhbox\derboxtwo\unhbox\derboxone}%
   \advance\derccdim by\derldim
   \advance\derccdim by\dercdim
           \dercrdim  =\derrdim
   \rootaux{#1}{#2}{#3}}%
\def\root       #1#2#3{\rootr  {#1\;}{\;}{#2}{#3}}%
\def\rroot    #1#2#3#4{\rrootr {#1\;}{\;}{#2}{#3}{#4}}%
\def\rrroot #1#2#3#4#5{\rrrootr{#1\;}{\;}{#2}{#3}{#4}{#5}}%
\def\rootnote #1#2#3#4{\rootr  {#1\;}{\;#2}{#3}{#4}}%

\newbox\stembox
\def\stemaux #1#2#3{\setbox\derboxtwo=\hbox{\unhbox\derboxone}%
                                                  % b2=b1
   \setbox\derboxthree=\hbox{$#1$}   % b3; l=wd(b3)
   \setbox\derboxfour =\hbox{$#2$}   % b4; m=wd(b4)
      {\global\setbox\derboxone=\hbox{$#3$}%
      \global\derldim=0pt                         % dl=0
      \global\dercdim=\wd\derboxone               % dc=wd(b1)
      \global\derrdim=0pt                         % dr=0
      }%                                          % dl=0, dc=wd(b1), dr=0
   \derdim=\dercdim\advance\derdim by-\derccdim\divide\derdim by2 
                                                  % d=(dc-dcc)/2
   \global\derldim=\dercldim\global\advance\derldim by-\derdim
                                                  % dl=dcl-d
   \global\derrdim=\dercrdim\global\advance\derrdim by-\derdim
                                                  % dr=dcr-d
   \deropen=\fontdimen5\textfont2\divide\deropen by3
   \setbox\derboxone=\hbox{\vbox{\offinterlineskip
         \hbox{\ifdim\derldim<0pt\kern-\derldim\fi
               \box\derboxtwo
               \ifdim\derrdim<0pt\kern-\derrdim\fi}%
         \kern-\deropen\kern-\ht\strutbox\kern-\dp\strutbox
         \hbox{\ifdim\dercldim>\derldim
                  \ifdim\derldim>0pt\kern\derldim\fi
                  \else\kern\dercldim\fi
               \hbox to0pt{\hss\copy\derboxthree}%
               \vbox{\ifdim\derccdim>\dercdim\hsize=\derccdim
                                        \else\hsize=\dercdim \fi
                    \hbox{$\vcenter{
                    \vbox{\offinterlineskip
                       \hbox{$\copy\stembox$}\kern-1\dp\stembox
                       \hbox{$\copy\stembox$}}}$}}%
               \hbox to0pt{\copy\derboxfour\hss}%
               \ifdim\dercrdim>\derrdim
                  \ifdim\derrdim>0pt\kern\derrdim\fi
                  \else\kern\dercrdim\fi}%
         \kern-\deropen
         \hbox{\ifdim\derldim>0pt\kern\derldim\fi
               \box\derboxone
               \ifdim\derrdim>0pt\kern\derrdim\fi}}}%
   \ifdim\derldim<0pt\global\derldim=0pt\fi       % dl=max(dl,0)
   \ifdim\derrdim<0pt\global\derrdim=0pt\fi       % dr=max(dr,0)
   \derdldim=\wd\derboxthree\advance\derdldim by-\dercldim
                                                  % ddl=l-dcl
   \derdrdim=\wd\derboxfour \advance\derdrdim by-\dercrdim
                                                  % ddr=m-dcr
   \ifdim\derdim<0pt
      \ifdim\derdldim<0pt
         \derdldim=0pt                            % d<0, ddl<0 -> ddl=0
      \fi
      \ifdim\derdrdim<0pt
         \derdrdim=0pt                            % d<0, ddr<0 -> ddr=0
      \fi
   \else
      \ifdim\derldim>0pt
         \ifdim\derdldim>-\derdim
            \advance\derdldim by\derdim           % d>=0, dl>0, ddl+d>0 -> 
         \else			                  %                    ddl=ddl+d
            \derdldim=0pt                         % d>=0, dl>0, ddl+d<=0 ->
         \fi                                      %                        ddl=0
      \else
         \advance\derdldim by\dercldim            % d>=0, dl=0 -> ddl=ddl+dcl
      \fi
      \ifdim\derrdim>0pt
         \ifdim\derdrdim>-\derdim
            \advance\derdrdim by\derdim           % d>=0, dr>0, ddr+d>0 -> 
         \else			                  %                    ddr=ddr+d
            \derdrdim=0pt                         % d>=0, dr>0, ddr+d<=0 ->
         \fi                                      %                        ddr=0
      \else
         \advance\derdrdim by\dercrdim            % d>=0, dr=0 -> ddr=ddr+dcr
      \fi
   \fi
   \global\setbox\derboxone=\hbox
      {\kern\derdldim\unhbox\derboxone\kern\derdrdim}%
   \global\advance\derldim by\derdldim            % dl=dl+ddl
   \global\advance\derrdim by\derdrdim            % dr=dr+ddr
   }%
\def\stemauxx #1#2#3{\setbox\derboxtwo=\hbox{\unhbox\derboxone}%
                                                  % b2=b1
   \setbox\derboxthree=\hbox{$#1$}   % b3; l=wd(b3)
   \setbox\derboxfour =\hbox{$#2$}   % b4; m=wd(b4)
   \leaf{#3}%                                     % dl=0, dc=wd(b1), dr=0
   \derdim=\dercdim\advance\derdim by-\derccdim\divide\derdim by2 
                                                  % d=(dc-dcc)/2
   \global\derldim=\dercldim\global\advance\derldim by-\derdim
                                                  % dl=dcl-d
   \global\derrdim=\dercrdim\global\advance\derrdim by-\derdim
                                                  % dr=dcr-d
   \deropen=\fontdimen5\textfont2\divide\deropen by3
   \setbox\derboxone=\hbox{\vbox{\offinterlineskip
         \hbox{\ifdim\derldim<0pt\kern-\derldim\fi
               \box\derboxtwo
               \ifdim\derrdim<0pt\kern-\derrdim\fi}%
         \kern\deropen
         \hbox{\ifdim\dercldim>\derldim
                  \ifdim\derldim>0pt\kern\derldim\fi
                  \else\kern\dercldim\fi
               \hbox to0pt{\hss\copy\derboxthree}%
               \vbox{\ifdim\derccdim>\dercdim\hsize=\derccdim
                                        \else\hsize=\dercdim \fi
                    \hbox{\hfil}}%
               \hbox to0pt{\copy\derboxfour\hss}%
               \ifdim\dercrdim>\derrdim
                  \ifdim\derrdim>0pt\kern\derrdim\fi
                  \else\kern\dercrdim\fi}%
         \kern\deropen
         \hbox{\ifdim\derldim>0pt\kern\derldim\fi
               \box\derboxone
               \ifdim\derrdim>0pt\kern\derrdim\fi}}}%
   \ifdim\derldim<0pt\global\derldim=0pt\fi       % dl=max(dl,0)
   \ifdim\derrdim<0pt\global\derrdim=0pt\fi       % dr=max(dr,0)
   \derdldim=\wd\derboxthree\advance\derdldim by-\dercldim
                                                  % ddl=l-dcl
   \derdrdim=\wd\derboxfour \advance\derdrdim by-\dercrdim
                                                  % ddr=m-dcr
   \ifdim\derdim<0pt
      \ifdim\derdldim<0pt
         \derdldim=0pt                            % d<0, ddl<0 -> ddl=0
      \fi
      \ifdim\derdrdim<0pt
         \derdrdim=0pt                            % d<0, ddr<0 -> ddr=0
      \fi
   \else
      \ifdim\derldim>0pt
         \ifdim\derdldim>-\derdim
            \advance\derdldim by\derdim           % d>=0, dl>0, ddl+d>0 -> 
         \else			                  %                    ddl=ddl+d
            \derdldim=0pt                         % d>=0, dl>0, ddl+d<=0 ->
         \fi                                      %                        ddl=0
      \else
         \advance\derdldim by\dercldim            % d>=0, dl=0 -> ddl=ddl+dcl
      \fi
      \ifdim\derrdim>0pt
         \ifdim\derdrdim>-\derdim
            \advance\derdrdim by\derdim           % d>=0, dr>0, ddr+d>0 -> 
         \else			                  %                    ddr=ddr+d
            \derdrdim=0pt                         % d>=0, dr>0, ddr+d<=0 ->
         \fi                                      %                        ddr=0
      \else
         \advance\derdrdim by\dercrdim            % d>=0, dr=0 -> ddr=ddr+dcr
      \fi
   \fi
   \global\setbox\derboxone=\hbox
      {\kern\derdldim\unhbox\derboxone\kern\derdrdim}%
   \global\advance\derldim by\derdldim            % dl=dl+ddl
   \global\advance\derrdim by\derdrdim            % dr=dr+ddr
   }%
\def\stemr #1#2#3#4{{#4}%
   \dercldim=\derldim
   \derccdim=\dercdim
   \dercrdim=\derrdim
   \stemaux{#1}{#2}{#3}}%
\def\stemrr #1#2#3#4{{#4}%
   \dercldim=\derldim
   \derccdim=\dercdim
   \dercrdim=\derrdim
   \stemauxx{#1}{#2}{#3}}%
\def\stem #1#2#3#4{\setbox\stembox=\hbox{$\|$}%
   \stemrr{  }{  }{#3              }  {
   \stemr {#1\;}{\;#2}{\kern\wd\stembox} {
   \stemrr{  }{  }{\kern\wd\stembox}{
   #4                             }}}}%
\def\stempr #1#2#3{\setbox\stembox=\hbox{$\|$}%
   \stemrr{  }{  }{#3              }  {
   \stemr {#1\;}{\;#2}{\kern\wd\stembox} {
   \stemrr{  }{  }{\kern\wd\stembox}{
      {\global\setbox\derboxone=\hbox{%
         \vbox to0pt{\vss\hbox{$-$}\vss\kern-2\deropen}}%
      \global\derldim=0pt                            % dl=0
      \global\dercdim=\wd\derboxone                  % dc=wd(b1)
      \global\derrdim=0pt                            % dr=0
      }                             }}}}%

\def\deraux {\derldim=0pt\dercdim=0pt\derrdim=0pt}%
\def\der       #1#2#3{\deraux\root  {#1}{#2}{#3}        \box\derboxone}%
\def\dder    #1#2#3#4{\deraux\rroot {#1}{#2}{#3}{#4}    \box\derboxone}%
\def\ddder #1#2#3#4#5{\deraux\rrroot{#1}{#2}{#3}{#4}{#5}\box\derboxone}%
\def\dernote       #1#2#3#4{\deraux\rootr  {#1\;}{\;#2}{#3}{#4}\box\derboxone}%
\def\ddernote    #1#2#3#4#5{\deraux\rrootr {#1\;}{\;#2}{#3}{#4}{#5}\box
                                                                   \derboxone}%
\def\dddernote #1#2#3#4#5#6{\deraux\rrrootr{#1\;}{\;#2}{#3}{#4}{#5}{#6}\box
                                                                   \derboxone}%


%  macros for inference rules --------------------------------------------------

% \newdimen\infopen
% \infopen=\fontdimen5\textfont2\divide\infopen by3
% \def\inflabel #1{\vbox to0pt{\vss\hbox{${#1}\;\mathstrut$}\vss}}%
% \def\inflabelnote #1{\vbox to0pt{\vss\hbox{$\;{#1}\mathstrut$}\vss}}%
% \def\infaux #1#2#3{\infopen=\fontdimen5\textfont2\divide\infopen by3
%         \vbox{\offinterlineskip\halign{##&\hfil##\hfil\cr
%         &\hbox{\strut$#3$}\cr
%         \noalign{\kern\infopen}%
%         \llap{\inflabel{#1}}&\cr
%         \noalign{\hrule}%
%         \noalign{\kern\infopen}%
%         &\hbox{\strut$#2$}\cr}}}%
% \def\infauxnote #1#2#3#4{\hbox
%    {\infopen=\fontdimen5\textfont2\divide\infopen by3
%       \vbox{\offinterlineskip\halign{##&\hfil##\hfil&##\cr
%          &\hbox{\strut$#3$}&\cr
%              \noalign{\kern\infopen}%
%              \llap{\inflabel{#1}}&&\rlap{\inflabelnote{#4}}\cr
%              \noalign{\hrule}%
%              \noalign{\kern\infopen}%
%          &\hbox{\strut$#2$}&\cr}}\phantom{\inflabelnote{#4}}}}%
% \def\inf #1#2#3{\hbox{\phantom{\inflabel{#1}}\infaux{#1}{#2}{#3}}}%
% \def\infnote #1#2#3#4{\hbox
%    {\phantom{\inflabel{#1}}\infauxnote{#1}{#2}{#3}{#4}}}%
% \def\infllap #1#2#3{\infaux{#1}{#2}{#3}}%
% \def\infllapnote #1#2#3#4{\infauxnote{#1}{#2}{#3}{#4}}%
% \def\iinf #1#2#3#4{\inf{#1}{#2}{#3\quad #4}}%
% \def\iinfnote #1#2#3#4#5{\infnote{#1}{#2}{#3\quad #4}{#5}}%
% \def\iinfllap #1#2#3#4{\infllap{#1}{#2}{#3\quad #4}}%
% \def\iiinf #1#2#3#4#5{\inf{#1}{#2}{#3\quad #4\quad #5}}%
% \def\iiinfnote #1#2#3#4#5#6{\infnote{#1}{#2}{#3\quad #4\quad #5}{#6}}%
\def\inf       #1#2#3{\der  {#1}{#2}{\leaf{#3}}}%
\def\iinf    #1#2#3#4{\dder {#1}{#2}{\leaf{#3}}{\leaf{#4}}}%
\def\iiinf #1#2#3#4#5{\ddder{#1}{#2}{\leaf{#3}}{\leaf{#4}}{\leaf{#5}}}%
\def\infnote       #1#2#3#4{\dernote  {#1}{#4}{#2}{\leaf{#3}}}%
\def\iinfnote    #1#2#3#4#5{\ddernote {#1}{#5}{#2}{\leaf{#3}}{\leaf{#4}}}%
\def\iiinfnote #1#2#3#4#5#6{\dddernote{#1}{#6}{#2}{\leaf{#3}}{\leaf{#4}}{\leaf
                                                                         {#5}}}%

\def\strpr  #1#2#3{\stempr{#1}{#2}{#3}\box\derboxone}%
\def\strder #1#2#3#4{\stem{#1}{#2}{#3}{#4}\box\derboxone}%

%  macro for skeleton derivations ----------------------------------------------

\newbox\derskelboxone
\newbox\derskelboxtwo
\newbox\derskelboxthree
\newbox\derskelboxfour
\newdimen\derskeldimenone
\newdimen\derskeldimentwo
\newdimen\derskeldimenthree
\newdimen\derskeldimenfour
\newdimen\derskeldimenfive
\newdimen\derskeldimensix
\newdimen\derskeldimenseven
\newdimen\derskeldimeneight
\def\derskel #1#2#3#4{%
   % left premise
   \setbox\derskelboxone=\hbox{$#1$\strut}%
   \derskeldimenone=\ht\derskelboxone
   \advance\derskeldimenone by\dp\derskelboxone
   \derskeldimentwo=\wd\derskelboxone
   \divide\derskeldimentwo by2
   \setbox\derskelboxone=\hbox to0pt{%
      \hss\raise\dp\derskelboxone\box\derskelboxone\hss}%
   \ht\derskelboxone=0pt
   \dp\derskelboxone=0pt
   % right premise
   \setbox\derskelboxtwo=\hbox{$#3$\strut}%
   \derskeldimenthree=\ht\derskelboxtwo
   \advance\derskeldimenthree by\dp\derskelboxtwo
   \derskeldimenfour=\wd\derskelboxtwo
   \divide\derskeldimenfour by2
   \setbox\derskelboxtwo=\hbox to0pt{%
      \hss\raise\dp\derskelboxtwo\box\derskelboxtwo\hss}%
   \ht\derskelboxtwo=0pt
   \dp\derskelboxtwo=0pt
   \ifdim\derskeldimenone>\derskeldimenthree
      \else\derskeldimenone=\derskeldimenthree\fi
   % conclusion
   \setbox\derskelboxthree=\hbox{$#4$\strut}%
   \derskeldimenfive=\ht\derskelboxthree
   \advance\derskeldimenfive by\dp\derskelboxthree
   \derskeldimensix=\wd\derskelboxthree
   \divide\derskeldimensix by2
   \setbox\derskelboxthree=\hbox to0pt{%
      \hss\lower\ht\derskelboxthree\box\derskelboxthree\hss}%
   \ht\derskelboxthree=0pt
   \dp\derskelboxthree=0pt
   % middle premises
   \setbox\derskelboxfour=\hbox{$#2$\strut}%
   \derskeldimenseven=\ht\derskelboxfour
   \advance\derskeldimenseven by\dp\derskelboxfour
   \derskeldimeneight=\wd\derskelboxfour
   \divide\derskeldimeneight by2
   \setbox\derskelboxfour=\hbox to0pt{%
      \hss\raise\dp\derskelboxfour\box\derskelboxfour\hss}%
   \ht\derskelboxfour=0pt
   \dp\derskelboxfour=0pt
   \ifdim\derskeldimenone>\derskeldimenseven
      \else\derskeldimenone=\derskeldimenseven\fi
   %
   \derskeldimenthree=\derskeldimentwo
   \advance\derskeldimenthree by2\derskeldimeneight
   \advance\derskeldimenthree by\derskeldimenfour
   \advance\derskeldimenthree by2em
   \divide\derskeldimenthree by2
   %
   \advance\derskeldimensix by-\derskeldimenthree
   \derskeldimenseven=\derskeldimensix
   \advance\derskeldimensix by-\derskeldimentwo
   \advance\derskeldimenseven by-\derskeldimenfour
   \ifdim\derskeldimensix>0pt
      \else\derskeldimensix=0pt\fi
   \ifdim\derskeldimenseven>0pt
      \else\derskeldimenseven=0pt\fi
   \vbox{\kern\derskeldimenone\hbox{\kern\derskeldimensix
         \kern\derskeldimentwo
         \xy
         <-\derskeldimenthree,\derskeldimenthree>="here"
            *{\box\derskelboxone}**\dir{-};
         "here"+<\derskeldimentwo,0pt>="here"**\dir{-};
         "here"+<1em,0pt>="here"**\dir{-};
         "here"+<\derskeldimeneight,0pt>="here"
            *{\box\derskelboxfour}**\dir{-};
         "here"+<\derskeldimeneight,0pt>="here"**\dir{-};
         "here"+<1em,0pt>="here"**\dir{-};
         "here"+<\derskeldimenfour,0pt>*{\box\derskelboxtwo}**\dir{-};
         0*{\box\derskelboxthree}**\dir{-};
         <-\derskeldimenthree,\derskeldimenthree>**\dir{-}
         \endxy
         \kern\derskeldimenfour\kern\derskeldimenseven}%
      \kern\derskeldimenfive}}%

